Diffusion Model for Planning: A Systematic Literature Review

Diffusion models, which leverage stochastic processes to capture complex data distributions effectively, have shown their performance as generative models, achieving notable success in image-related tasks through iterative denoising processes. Recently, diffusion models have been further applied and show their strong abilities in planning tasks, leading to a significant growth in related publications since 2023. To help researchers better understand the field and promote the development of the field, we conduct a systematic literature review of recent advancements in the application of diffusion models for planning. Specifically, this paper categorizes and discusses the current literature from the following perspectives: (i) relevant datasets and benchmarks used for evaluating diffusion modelbased planning; (ii) fundamental studies that address aspects such as sampling efficiency; (iii) skill-centric and condition-guided planning for enhancing adaptability; (iv) safety and uncertainty managing mechanism for enhancing safety and robustness; and (v) domain-specific application such as autonomous driving. Finally, given the above literature review, we further discuss the challenges and future directions in this field.

==> biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author_photo/author_ubu.jpg}}]{Toshihide Ubukata}
    is now a master student at Waseda University in Tokyo, Japan.
    He received B.E in Computer Science from Waseda University in 2024. 
    His research interests are in self-adaptive systems, autonomous agent system.
    He is a member of the IEEE Computer Society (IEEE CS).
\end{IEEEbiography}


\vspace{-3mm}



\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author_photo/author_li.png}}]{Jialong Li}
    is now a research associate at Waseda University in Tokyo, Japan.
    He received B.E and M.E degrees in Computer Science from Waseda University in 2019 and 2021. 
    His research interests are in self-adaptive systems, software engineering, and human-computer interaction.
    He is a member of the IEEE Computer Society (IEEE CS), and Association for Computing Machinery (ACM).
    He has served Program Committee of International Conference on Software Engineering for Adaptive and Self-Managing Systems (SEAMS).
\end{IEEEbiography}


\vspace{-3mm}

    
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author_photo/author_tei.jpg}}]{Kenji Tei}
    is an associate professor at Tokyo Institute of Technology.
    He is also an associate professor by special appointment of National Institute of Informatics (NII).
    He is interested in self-adaptive software, software architecture, model-driven engineering, and software veriﬁcation.
    He is a member of the IEEE Computer Society (IEEE CS), Association for Computing Machinery (ACM), Information Processing Society of Japan (IPSJ), and Institute of Electronics, Information and Communication Engineers (IEICE).
    He currently serves Associate Editor of ACM Transactions on Autonomous and Adaptive Systems (TAAS).
    He has served Steering Committee Member of International Symposium on Software Engineering for Adaptive and Self-Managing Systems (SEAMS) and Program co-Chair of SEAMS ’19.
\end{IEEEbiography}

